On minimum phase transformation and filter design

Minimum-phase finite impulse response filters are widely used in practice, and much research has been devoted to the design of such filters. However, for the important case of Chebyshev filters there is a curious mismatch between current best practice and well-established theoretical principles. The paper shows that this difference can be understood through analysis of the time-domain factorization of a suitable extended matrix. This analysis explains why the definition of a factorable linear phase filter must be revised. The time domain analysis of factorization suggests initial values leading to fast and accurate convergence of iterative algorithms for the design of minimum-phase finite impulse response filters. Numerical results are provided to demonstrate that a significant improvement in filter tap accuracy is obtained when the well-established theoretical principles are correctly applied to the design of minimum phase finite impulse response filters.

==> mybibfile.tex <==
@book{linear_syst,
  author =        {T. ~Kailath},
  publisher =     {Prentice-Hall},
  series =        {},
  title =         {Linear Systems},
  year =          {1980},
}

@ARTICLE{poor,  author={K. {Vastola} and H. {Poor}},  journal={IEEE Transactions on Information Theory},   title={Robust Wiener-Kolmogorov theory},   year={1984},  volume={30},  number={2},  pages={316-327},  doi={10.1109/TIT.1984.1056875}}

@article{cioffi,
  author={N Al-Dhahir and J.M. Cioffi},
  journal={IEEE Transactions on Information Theory}, 
  title={{MMSE} decision-feedback equalizers: finite-length results}, 
  year={1995},
  volume={41},
  number={4},
  pages={961-975},
  doi={10.1109/18.391242}}

@book{oppenheim,
  author =        {A.~V. Oppenheim and R.~W. Schafer},
  publisher =     {Pearson Education},
  series =        {},
  title =         {Digital Signal Processing},
  year =          {2015},
}

@book{oppenheim2,
  author =        {A.~V. Oppenheim and R.~W. Schafer},
  publisher =     {Prentice-Hall},
  series =        {},
  title =         {Discrete-Time Signal Processing},
  year =          {1989},
}

@book{smith,
  author =        {Smith},
  publisher =     {},
  series =        {},
  title =         {Introduction to Digital Filters with Audio Applications},
  year =          {},
    url =           { https://ccrma.stanford.edu/jos/},
}

@book{proakis2,
  author =        {J.~G. Proakis and D.~G. Manolakis},
  publisher =     {New York: Macmillan},
  series =        {},
  title =         {Digital signal processing: Principles, algorithms, and applications},
  year =          {1992},
}

@book{proakis1,
  author =        {J.~G. Proakis and M. Salehi},
  publisher =     {Boston: McGraw-Hill},
  series =        {},
  title =         {Digital Communications},
  year =          {2008},
}


@book{linear_est,
  author =        {T. ~Kailath and A.~H. Sayed and B. Hassibi},
  publisher =     {Upper Saddle River, N.J., Prentice Hall},
  series =        {},
  title =         {Linear Estimation},
  year =          {2000},
}

@book{kalman,
  author =        {B. Ristic and  S.  Arulampalam},
  publisher =     {Boston, MA, Artech House},
  series =        {},
  title =         {Beyond the Kalman filter: particle filters for tracking applications},
  year =          {2004},
}



@article{o-w,
  author =        {H. ~J. Orchard and A. ~N Wilson},
  journal =       {IEEE Trans. Circuits Syst. I, Fundam. Theory Appl.},
  pages =         {365--375},
  title =         {On the computation of a minimum phase spectral factor},
  volume =        {50},
  year =          {2003},
}

@article{antonio,
  author =        {S. Kidambi and A. Antoniou},
  journal =       {IEEE Trans. Circuits and Systems -- II: Express briefs},
  pages =         {472--476},
  title =         {Design of Minimum-Phase Filters Using Optimization},
  volume =        {64},
  year =          {2017},
}

@article{parks,
  author =        {L. ~R. Rabiner and J.~H. McClellan and T. ~W. Parks},
  journal =       {Proceedings of the IEEE},
  pages =         {595--610},
  title =         {FIR Digital Filter Design Techniques Using Weighted Chebyshev Approximation},
  volume =        {63},
  year =          {1975},
}

@article{evans,
  author =        {N. ~D. Venkata and B.~L. Evans and S. ~R. McCaslin},
  journal =       {IEEE Trans. Signal Process.},
  pages =         {1491--1495},
  title =         {Design of optimal minimum-phase digital FIR filters using discrete Hilbert transforms},
  volume =        {48},
  year =          {2000},
}

@article{herrmann,
  author =        {O. Herrmann and H.~W. Schuessler},
  journal =       {Electron. Lett.},
  pages =         {329--330},
  title =         {Design of non-recursive digital filters
with minimum phase},
  volume =        {6},
  year =          {1970},
}

@article{kamp,
  author =        {Y. Kamp and C.~J. Wellekens},
  journal =       {IEEE Trans. Acoust., Speech, Signal Process.},
  pages =         {922--926},
  title =         {Optimal design of minimum-phase FIR filters},
  volume =        {31},
  year =          {1983},
}


@article{reddy,
  author =        {G. ~R. Reddy},
  journal =       {Electron. Lett.},
  pages =         {1225--1227},
  title =         {Design of minimum-phase FIR digital filter through cepstrum},
  volume =        {22},
  year =          {1986},
}

@book{linear_alg,
  author =        {G. ~H. Golub and  C. ~F. {Van Loan}},
  publisher =     {},
  series =        {},
  title =         {Matrix Computations},
  year =          {2013},
}

@misc{regular,
  title = {Regularization},
  howpublished = {\url{https://math.stackexchange.com/questions/3596910/regularization-of-a-matrix-using-a-diagonal-matrix}},
  note = {Accessed: 2021-09-21}
}

@article{vainio,
  author =        {O. ~Vainio},
  journal =       {IEEE Trans. Instrum. Meas.},
  pages =         {1100--1102},
  title =         {Minimum-phase FIR filters for delay-constrained noise reduction},
  volume =        {48},
  year =          {1999},
}

@article{optics,
author = {Halir, Robert and Molina-Fernández, Iñigo and Wangüemert-Pérez, J and Ortega-Moñux, Alejandro and de-Oliva-Rubio, J. and Cheben, Pavel},
year = {2009},
month = {06},
pages = {8349-61},
title = {Characterization of integrated photonic devices with minimum phase technique},
volume = {17},
journal = {Optics express},
doi = {10.1364/OE.17.008349}
}

@ARTICLE{saltz,
  author={Salz, J.},
  journal={The Bell System Technical Journal}, 
  title={Optimum mean-square decision feedback equalization}, 
  year={1973},
  volume={52},
  number={8},
  pages={1341-1373},
  doi={10.1002/j.1538-7305.1973.tb02023.x}}



